Analysis of a blockchain protocol based on LDPC codes

In a blockchain Data Availability Attack (DAA), a malicious node publishes a block header but withholds part of the block, which contains invalid transactions. Honest full nodes, which can download and store the full blockchain, are aware that some data are not available but they have no formal way to prove it to light nodes, i.e., nodes that have limited resources and are not able to access the whole blockchain data. A common solution to counter these attacks exploits linear error correcting codes to encode the block content. A recent protocol, called SPAR, employs coded Merkle trees and low-density parity-check codes to counter DAAs. In this paper, we show that the protocol is less secure than claimed, owing to a redefinition of the adversarial success probability. As a consequence we show that, for some realistic choices of the parameters, the total amount of data downloaded by light nodes is larger than that obtainable with competitor solutions.

==> old.tex <==
Note that, to obtain vectors as in the above Lemma, it is enough to first choose $\6e$ at random.
Let $i$ be the position such that $e_i\neq 0$.
We then compute the indexes of the unsatisfied parity-check equation and, for each equation, pick an index $j\neq i$.
These positions correspond to the positions of the erasures we put in $\6e'$.
Note that, in case the same symbol participates in multiple equations, the number of erasures we need is lower than $v$.
\textcolor{red}{[Qui metterei una descrizione a parole del significato del lemma, magari una figura e rimanderei alla sezione seguente la spiegazione di come evitare l'attacco. A sto punto, attaccherei con il caso di multiple errors.]}
Let us suppose that the malicious full node introduces one Hamming error in the codeword of a $(v,w)$-regular LDPC code. This Hamming error makes incorrect (at most) $v$ parity-check equations defined by the LDPC code parity-check matrix. Then, the malicious full node computes the Merkle root based on the incorrect codeword. Then, in order to mask the incorrectness of these parity check equations, the malicious full node also introduces erasures in the codeword, in such a way that each of the incorrect parity check equation contains at least an erasure. We can assume that the malicious node introduces the minimum number of erasures $\epsilon^*$ achieving this goal, in order to minimize the probability that light node asks for an erased symbol in the sampling procedure. Due to the randomness in the code construction, and to the slight irregularity of the considered codes, $\epsilon^*$ cannot be determined a priori. Eventually, the malicious node broadcasts the block with missing (and corrupted) data.

From a light node perspective, there is no qualitative difference between the classical and the novel attack, since it does not download the coded Merkle tree and is not able to recognize either erasures or errors. Moreover, even if during the sampling procedure light nodes catch an erred symbol, they cannot verify whether the parity-check equations it belongs to are verified, but can only verify if they match the correct Merkle root. The latter condition is indeed verified, since the malicious node has computed the Merkle root based on the erroneously coded Merkle tree. 

Therefore, also in this situation, honest full nodes should find a way to prove to light nodes that a data availability attack is going on. Differently from the case where symbols are only hidden (\emph{i.e.}, erased), the hash-aware peeling decoder fills the erasures, but it performs it incorrectly in the parity check equations containing also the erred symbol. Eventually, honest full nodes need to find at least a pair of parity-check equations in which the same erased symbol assumes two different values or, in other words, a parity check equation which becomes unsatisfied do to the introduced error. Let us analyze this scenario formally.

Let $\6c$ be a codeword of length $n$ obtained by encoding $\6u$ of length $k$. Then, we have that $\6x=\6c+\6e+\6e'$, where $\6e$ is the vector containing errors (and therefore takes values in $\mathbb F_q$), and $\6e'$ is a vector containing erasures (and therefore takes values in $\{0,\epsilon\}$, where $\epsilon$ is the symbol denoting an erasure). As anticipated, let us consider
\[
w_\mathrm{H}(\6e) = 1,
\]
that is, a single erred symbol is introduced by the adversary.


We can stick to the case where, for at least a value of $i$, \eqref{eq:supperrori} holds with equality sign, and generalize it later in this section.

 Notice that finding a set of symbols such that (at most) $c$ parity check equations contain one erasure can be done in polynomial time. This way, a honest full node will recover the erasures incorrectly, but cannot prove it to light nodes by broadcasting a single parity check equation and the corresponding Merkle proofs. In fact, due to the malicious node strategy, any single incorrect parity-check equation contains at least one erasure and, since the honest full node (and therefore the light nodes) recovers it incorrectly, the verification, even in presence of a Merkle proof for that symbol, is impossible for light nodes, since the Merkle root is computed with the incorrect symbol. %Still, there is a way out: the honest full node must find a pair of parity-check equations which prove the incorrectness of one them, along with the Merkle proofs of all the symbols in these parity check equations, except for the erased one. This way, the light nodes can locally  verify the mismatch between the values of the same erased symbol. %, or verify the mismatch between the downloaded Merkle root and the locally computed one.

Let us now provide an upper bound on the value of $\epsilon^*$.

\begin{Lem}
If a malicious full node has introduced a symbol error in a codeword of an LDPC code constructed according to \cite{yu2020coded}, the minimum number of erasures it needs to introduce so that each parity-check equation to which the symbol participates contains at least an erasure $\epsilon^*\leq c$.
\label{lemma11}
\end{Lem}
\begin{IEEEproof}
The upper bound is simply obtained by considering that the codes designed as in \cite{yu2020coded} have at most column weight $c$. Then, $\epsilon^*$ assumes its largest value when the erred symbols participates to exactly $c$ parity-check equations, and it is the only common symbol between them.
\end{IEEEproof}

%It is shown in Section \ref{subsec:ldpccodes} that the design of LDPC codes for SPAR provides irregular codes, with a parity-check matrix having column weight smaller than or equal to $c$, and row weight smaller than or equal to $d$. We conservatively assume that the malicious full node corrupts with an error a symbol which belongs to exactly $c$ parity-check equations. Moreover, we conservatively assume that the erred symbol is the only common symbol between the considered $c$ parity-check equations. In this scenario, in order to have exactly one erasure in each of the considered $c$ parity-check equations, it must be $\epsilon^*=c$. Clearly, we should consider this as an upper bound. In fact, if the erred symbol participates to less than $c$ parity check equations, say $c'\leq c$, then under the second assumption above, the number of hidden symbols is $\epsilon^*=c'$. Moreover, if the symbol participates to exactly $c$ parity check equations, but there are two or more common symbols belonging to the $c$ considered parity-check equations, the malicious full node could erase them, obtaining  $\epsilon^*<c$. Therefore, it must be $\epsilon^*\leq c$. An important remark is that $\epsilon^*$ does not depend on the code blocklength.

Let us now analyze the amount of data that honest full nodes must send to light nodes in order to proof the incorrect-coding fraud. 

\begin{Lem}
If the malicious full node introduces an error in the codeword of an of an LDPC code  constructed according to \cite{yu2020coded}, and introduces at least an erasure in each of the parity-check equations to which the symbol participates, an incorrect coding proof must contain at least:
\begin{itemize}
\item the value of the $d-1$ known symbols, along with their Merkle proofs, which belong to a satisfied parity-check equation containing a single erasure, let us say in the $i$th symbol.
\item the value of the $d-1$ known symbols (one of which is incorrect), along with their Merkle proofs, which belong to an unsatisfied parity-check equation containing an erasure of the $i$th symbol. 
\end{itemize}
\end{Lem}
\begin{IEEEproof}
The minimal content of the fraud proof is obtained conservatively assuming that there exists a corrupted parity-check equation containing only one erasure and, in the worst case scenario for the adversary, that there exist a correct parity-check equation containing only one erasure, on the same symbol of the corrupted one. These two parity-check equations assign two different values to the same erasure, because one of them is correct and one of them is not. 
\end{IEEEproof}

The situation complicates if, instead of erasing one symbol per corrupted parity-check equation, the malicious full node erases at least $v_{\epsilon}$ symbols per corrupted parity-check equation, that is,
\begin{equation}
  |\mathrm{supp}(\6e') \cap \mathrm{supp}(\6H_{i,:}) | \geq v_{\epsilon}, \hspace{1pt} \forall i \in E,  
  \label{eq:supperrori2}
\end{equation} 
where, again, we assume that there exists at least an $i$ for which \eqref{eq:supperrori2} holds with equality sign (this is the worst case for the adversary). 
\begin{Cor}
If a malicious full node has introduced a symbol error in a codeword of an LDPC code constructed according to \cite{yu2020coded}, the minimum number of erasures it needs to introduce so that each parity-check equation to which the symbol participates contains at least $v_{\epsilon}$ erasures is smaller than or equal to $\min(v_{\epsilon}c,n-1)$.
\end{Cor}
\begin{IEEEproof}
Similar to the proof of Lemma \ref{lemma11}.
\end{IEEEproof}

The effect of the above result is then twofold: on the one hand, the number of symbols the adversary needs to erase increases, that is, the size of the $|\mathrm{supp}(\6e')|$ increases, facilitating the sampling procedure by light nodes; on the other hand, full nodes cannot prove anymore the fraud only using a pair of parity-check equations (along with the Merkle proofs of the known symbols participating to them). 

\begin{Lem}
If the malicious full node introduces an error in the codeword of an of an LDPC code  constructed according to \cite{yu2020coded}, and introduces at least $v_{\epsilon}$ erasures in each of the parity-check equations to which the symbol participates, an incorrect coding proof must contain at least:
\begin{itemize}
\item the value of the at the $d-v_{\epsilon}$ known symbols (one of which is incorrect), along with their Merkle proofs, which belong to an incorrect parity-check equation containing $v_{\epsilon}$ erasures.
\item the value of at most $v_{\epsilon}(d-1)$ known symbols, along with their Merkle proofs, which belong to the $v_{\epsilon}$ parity-check equations allowing to recover the erased symbols of the above incorrect parity-check equation and to prove that a discrepancy is present (in particular, $v_\epsilon-1$ parity-check equations to fill the erasures and a correct one to prove the discrepancy). 
%$\frac{2dv_{\epsilon}-v_{\epsilon}^2+v_{\epsilon}-2}{2}$ and
\end{itemize}
\end{Lem}
\begin{IEEEproof}
In order to find the content of a fraud proof under the above assumptions, we have conservatively considered that an incorrect parity-check equation with the minimal number of erasures exists. This justifies the first point of the list.

Then, honest full nodes need to recover these $v_{\epsilon}$ erasures, and at least $v_{\epsilon}-1$ equations are needed for this. Considering that each parity-check equation contains at most $d$ symbols, the maximum number of known symbols to be included in the proof is $(v_{\epsilon}-1)(d-1)$, having assumed that each of the $v_{\epsilon}-1$ equations only contains an erasure. Then, another correct parity-check equation must be included in the proof, in order to prove the mismatch, which requires  at most $d-1$ more known symbols. %The minimum number of known symbols to be included in the proof is obtained if there is a parity-check equation containing only $1$ erasure, one containing only $2$ erasures, and so on, up to $d-(v_{\epsilon}-1)$ erasures. The total number of known symbols in the proof is then at least $(\sum_{i=1}^{v_\epsilon-1}d-i)+(d-1)=\frac{2dv_{\epsilon}-v_{\epsilon}^2+v_{\epsilon}-2}{2}$, where the $(d-1)$ term is again the number of known symbols of the correct parity-check equation which must be included to prove the mismatch. 
\end{IEEEproof}
Notice that, once again, we have considered the worst case scenario for the adversary, that is, we have assumed that a set of correct equations allowing to recover these erasures exist, which might not always be the case. 

If $v_{\epsilon}$ is sufficiently large, or if the adversary is (computationally) strong enough to find stopping sets, our attack coincides with that considered in \cite{yu2020coded}. When a stopping set is erased the honest full nodes have no way of recovering the erasures and cannot provide an incorrect proof. The mechanism to be followed is different in this situation, and it is based on the so-called \emph{bad-coding} proofs \cite{yu2020coded}. 
%We remark that this is not the only strategy the malicious nodes can use to impede successful decoding to honest full nodes. For example, another sufficient condition to achieve this goal is that $\6e'$ has non-zero entries on positions corresponding to a stopping set. Still, searching for short stopping sets of LDPC codes designed as described in Section \ref{subsec:ldpccodes} is NP-hard, and therefore the attacker may not be able to find them. Moreover, as we shall see in the following section, the number of symbols to be erased when erasing a stopping set is way larger than that resulting from our attack.

\subsection{General scenario: multiple Hamming errors}

 The above discussion can be formally generalized to the case of 
\[
w_\mathrm{H}(\6e) = w_e\geq1.
\]
Let us consider the linear system containing the $r$ parity-check equations defined by the code parity-check matrix; recalling that $\6x=\6c+\6e+\6e'$, we have that
\begin{equation}
    \begin{cases}
      \6H_{1,1}x_1+\6H_{1,2}x_2+\ldots+\6H_{1,n}x_n=0,\\
     \6H_{2,1}x_1+\6H_{2,2}x_2+\ldots+\6H_{2,n}x_n=0,\\
     \vdots \\
     \6H_{r,1}x_1+\6H_{r,2}x_2+\ldots+\6H_{r,n}x_n=0.\\
    \end{cases}
    \label{eq:linsys}
    \end{equation}
Let also $w_\mathrm{H}(\6e') = w_\epsilon$;
the $w_\epsilon$ erasures introduced by the adversary can be seen as the unknowns of the above linear system, which is overdetermined for $w_{\epsilon}<r$. Under the assumption that $\6e$ and $\6e'$ have disjoint supports ($e_i=0$, $\forall i \in\mathrm{supp}(\6e') $), the following holds
\[
\sum_{j\in \mathrm{supp}(\6e')} x_j \6H_{:,j} = - \sum_{i\not\in \mathrm{supp}(\6e')} {(e_i+c_i)\6H_{:,i}}.
\]
Being $\6H$ public and $e_i+c_i$ known $\forall i$, the peeling decoder needs to solve the above parity-check equations, where we have separated the contributions due to  erasures (right hand side) and to errors (left hand side).

From an adversarial point of view, we study the case for which  $w_{\epsilon}<r$, that is, the system is overdetermined, and may be consistent (it admits solutions), or inconsistent (it admits no solution). 

\begin{Lem}
Given that $w_e\geq 1$ and that $\6e$ and $\6e'$ have disjoint supports, if  $\6c+\6e$ is a codeword, then the linear system defined by \eqref{eq:linsys} is consistent.
\label{lem:codeword}
\end{Lem}
\begin{IEEEproof}
By the Rouché-Capelli theorem, the linear system defined by \eqref{eq:linsys} is consistent if and only if the rank of $\6H_{:,\mathrm{supp}(\6e')}$ is equal to the rank of 
\[
[\6H_{:,\mathrm{supp}(\6e')} | - \6H_{:,[1,n]/ \mathrm{supp}(\6e')}\cdot(\6e+\6c)_{[1,n]/ \mathrm{supp}(\6e')}^\top ].
\]
If $\6c+\6e$ is a codeword (necessarily different from $\6c$, being $w_e\geq 1$, meaning that $\6e$ is a codeword), then by definition
\[\6H_{:,[1,n]/ \mathrm{supp}(\6e')}\cdot(\6e+\6c)_{[1,n]/ \mathrm{supp}(\6e')}^\top=0,\]
which proves the thesis. 
\end{IEEEproof}


\begin{comment}
Having assumed that $w_e\geq 1$, the only possibility for consistency is that $\6c+\6e$ is a codeword, different from the original one. Formally, it holds that
\[
\sum_{j'\not\in \mathrm{supp}(\6e')} {(e_{j'}+c_{j'})\6H_{:,j'}}+\sum_{j''\in \mathrm{supp}(\6e')} {(e_{j''}+c_{j''})\6H_{:,{j''}}}=0, 
\]
from which
\[
\sum_{j\in \mathrm{supp}(\6e')} x_j \6H_{:,j} = \sum_{i\in \mathrm{supp}(\6e')} {(e_i+c_i)\6H_{:,i}}=0,
\]
which is the definition of codeword. 
\end{comment}


Therefore, in this case, in order to prove the fraud to light nodes, honest full nodes need to forward them the Merkle proofs of all the information symbols. 


\begin{Cor}
Given that $w_e\geq 1$ and that $\6e$ and $\6e'$ have disjoint supports, then the linear system defined by \eqref{eq:linsys} is inconsistent if and only if  the rank of $\6H_{:,\mathrm{supp}(\6e')}$ is smaller than the rank of 
\[
[\6H_{:,\mathrm{supp}(\6e')} | - \6H_{:,\mathrm{supp}(\6e)}\cdot\6e_{\mathrm{supp}(\6e)}^T ].
\]
\label{cor:corcap}
\end{Cor}
\begin{IEEEproof}
If $\6c+\6e$ is a codeword, we have proved in Lemma \ref{lem:codeword} that the system is consistent. If, instead, $\6c+\6e$ is not a codeword, we can only state that
\[
\sum_{j\in[1,n]} {c_{j}\6H_{:,{j}}}=0, 
\]
from which
\[
\sum_{j\in \mathrm{supp}(\6e')} x_j \6H_{:,j} = - \sum_{i\not\in \mathrm{supp}(\6e')} {e_i\6H_{:,i}}+\sum_{j\in \mathrm{supp}(\6e')} {c_j\6H_{:,j}}.
\]
Considering that there are no errors in the positions indexed by the support of $\6e'$, we have that
\[
\sum_{j\in \mathrm{supp}(\6e')} e'_j \6H_{:,j} = - \sum_{i\not\in \mathrm{supp}(\6e')} {e_i\6H_{:,i}}= - \sum_{i\in \mathrm{supp}(\6e)} {e_i\6H_{:,i}}.
\]
The resulting linear system is then inconsistent if  the rank of $\6H_{:,\mathrm{supp}(\6e')}$ is smaller than the rank of 
\[
[\6H_{:,\mathrm{supp}(\6e')} | - \6H_{:,\mathrm{supp}(\6e)}\cdot\6e_{\mathrm{supp}(\6e)}^\top ].
\]

\end{IEEEproof}

So, Corollary \ref{cor:corcap} defines a condition the malicious full node can aspire to, in order to have guarantees that the peeling decoder will fail. 

Given this, we can now ask ourselves what is the worst case scenario for light nodes (in terms of downloaded data) and if the fact of having more than one Hamming error has an impact. We remark that, in order to just prove a fraud, it is sufficient for the full nodes to show that the same erased symbol assumes two different values. In order to just do this, it can exploit a correct parity-check equation and an incorrect parity-check equation. This is independent of the number of Hamming errors introduced by the malicious full nodes. Therefore, just from the standpoint of downloaded data, the number of introduced Hamming errors has no impact, as long as it is larger than zero.


==> spar.tex <==
The SPAR protocol is based on a novel hash accumulator called Coded Merkle Tree (CMT), combined with an ad-hoc  \textit{hash-aware} peeling decoder, which exploits the CMT structure to decode a codeword affected by erasures and, at the same time, checks for hash consistency.
We first briefly recall how these two algorithms operate, and then proceed by describing the SPAR protocol.

\subsection{Coded Merkle Tree}

A CMT is an hash accumulator which is constructed from $\ell$ linear codes $\{\code_1, \cdots,\code_\ell\}$ with ambient space $\mathbb F_q$; the $i$-th code has length $n_i$ and dimension $k_i$.
All the employed codes are implemented via systematic encoders, consequently we represent each $\code_i$ by the systematic parity-check matrix $\6H^{(i)}=[ \6A_i \hspace{0.5mm}|\hspace{0.5mm} \6I_{(n-k_i)}]$, with $\6A_i\in\mathbb F_q^{(n-k_i)\times k_i}$ and where $\6I_{(n-k_i)}$ is the identity matrix of size $n-k_i$. 
The CMT works with an integer $b$ which must be a divisor of all blocklength values $n_1,\cdots,n_\ell$.
Furthermore, one needs to have partitions for the sets $[1 ; n_i]$, for $i \in [1 , \ell-1]$.
Namely, we have $\mathcal S_i = \left\{S_1^{(i)},\cdots,S_{k_{i+1}}^{(i)}\right\}$ which is a partition of $[1 ; n_i]$, such that the $S_j^{(i)}$ are all disjoint and contain $b$ elements.
Starting from a codeword $\6c^{(1)}\in\code_1$, we build the associated CMT $\cmt(\6c)$ as follows:
\begin{enumerate}
    \item set $i = 1$;
    \item set $u_j = \hash\left(c^{(i)}_{z_1}|\cdots|c^{(i)}_{z_b}\right)$, where $\{z_1,\cdots,z_b\} = S^{(i)}_j$;
    \item encode $\6u = [u_1,\cdots,u_{k_{i+1}}]$ using $\6c^{(i+1)} (\6H^{(i)})^\top=\60$, where $\6c^{(i+1)}=[u_1,\cdots,u_{k_{i+1}} | c_{k_{i+1}+1},\cdots,c_{n_{i+1}}]$;
    \item if $i<\ell-1$, increase $i$ and restart from step 2), otherwise set $\cmtroot(\6c) = \6u$.
\end{enumerate}
%considering the following  First, we assume that each leaf is at the first layer (which we number as $1$); the data symbols of a layer are computed as the hash of the coded symbols of its child layer. Using a systematic code of rate $r$, at the lower level $n$ coded symbols are obtained from $k$ data symbols. Then, $b$ symbols are hashed and their hashes grouped into a data symbol, so that the data symbols of the successive layer are $\frac{n}{b}$. These symbols are then encoded with a different code (same rate but smaller $k$), and so on, until a layer with $t$ hashes is obtained, where $t\geq 1$. These $t$ hashes form (part of) the CMT root, $\mroot (\6c)$. Clearly, it must be $br>1$, or the process does not converge. 
\begin{comment}
\begin{figure*}[ht!]
    \centering
    \input{Figures/cmt2}
    \caption{Example of coded Merkle tree, for unspecified values of $n$ and $k$.}
    \label{fig:my_label}
\end{figure*}
\end{comment}

%A graphical representation of this procedure is given in Figure \ref{fig:my_label}.
The Merkle proof of any symbol in the CMT consists of the sibling hashes between the symbol and the Merkle root considering that, in each layer, each symbol has $b-1$ sibling hashes. % Then, aAny light node samples $s$ coded symbols in the base layer, along with their Merkle proofs. Due to the structure of the Merkle tree, this results in automatically sampling $s$ data symbols from each intermediate layer. Then, $(1-R_i)s$ extra symbols are sampled probabilistically from each intermediate layer. 

\subsection{Hash-aware peeling decoder}


An hash aware peeling decoder is an algorithm that decodes a tuple of $\ell$ codeword which are expected to constitute a CMT, in case they are affected by erasures.
Namely, let $\{\6x^{(1)},\cdots,\6x^{(\ell)}\}$, where $\6x^{(i)} = \6c^{(i)}+\6e'$, with $\6c^{(i)}\in\code_i$ and $\6e'\in\{0,\epsilon\}^n$.
This decoder works in a top-down fashion and, at every iteration, uses the peeling decoder strategy (\ie, recover erasures that participate in univariate parity-check equations) for any layer of the CMT.
As the symbols are recovered, their consistency is checked via hash functions.
Similarly to the standard peeling decoder, decoding fails whenever a stopping set or an unsatisfied parity-check is met; furthermore, the hash aware peeling decoder fails in case check consistency fails for some layer.
\begin{comment}
The decoding procedure is, instead, interrupted if:
\begin{itemize}
    \item a decoded symbol does not match its hash;
    \item a decoded symbol fails one or more parity-check equations; 
    \item the malicious node has erased a stopping set, and therefore the  peeling decoder gets stuck.
\end{itemize}
If this happens, for each of these cases, honest full nodes should be able to provide an \emph{incorrect coding proof} to the connected light nodes, which can be informally defined a proof that a fraud in the coding procedure was attempted.
\textcolor{red}{??? Riusciamo a non parlare dei nodi qui?}
\end{comment}
% In this paper we focus on the second situation, when induced by . \textcolor{red}{[L'ho separato dalla sezione precedente. La sezione è incompleta, magari completiamola in un secondo momento. Comunque, io qua non direi nulla di malicious nodes eccetera, descriverei solamente l'algoritmo e quando e come ritorna una failure.]}

\subsection{SPAR (TITOLO)  DAAs}\label{subsec:spadaa}


In SPAR, the CMT is instantiated using the design procedure considered in \cite{Luby}, which leads to LDPC codes whose parity-check matrices have at most column weight $v$ and at most row weight $w$. 
The protocol makes use of another hash accumulator, which we will denote by $\merkle$ and which can be a simple Merkle tree.
Let $\6u\in\mathbb F_q^k$ denote the list of transactions. 
Then, an honestly constructed header contains $h_u = \mroot(\6u)$ and $h_c = \cmtroot(\6c)$, with $\6c$ being the encoding of $\6u$ through $\code_1$.

The authors of SPAR provide an analysis of the ASP of DAAs.
They focus on two situations:
\begin{enumerate}
    \item[a) ] if $\6c\not\in\code_1$, then the incorrect coding proof can be proving that a parity-check equation is not satisfied.
    \item[b) ] if $\6c = \6u\6G_1$ but $f(\6u) = {\sf{False}}$, the adversary succeeds only if the samples received by the oracle are not enough to allow for the decoding of $\6c$;
\end{enumerate}
The authors of SPAR basically consider only proofs of type b) to study the ASP of DDAs, and claim the following bound for the ASP \cite[Theorem 1]{yu2020coded}:
\begin{equation}
\gamma \leq \min\left\{(1-\alpha_{min})^s\hspace{2mm},\hspace{2mm}2^{\max_{i}\{b(\alpha_i)n_i+ms\log(1-\alpha_i)\}}\right\},    
\end{equation}
where $b$ is the binary entropy function, $\alpha_i$ is the maximum number of \textcolor{red}{[Come le avevamo chiamate che non me lo ricordo?]}, $\alpha_{min} = \min_{i}(\alpha_i)$ and $s$ is the number of queries performed by each light node.
\textcolor{red}{[Diamo qualche numero?]}
% but, first, in the following section we give a formal definition of incorrect coding proof.

%, in which case an incorrect-coding proof can be forwarded to light nodes

\begin{comment}
\section{Incorrect coding proofs}

\textcolor{cyan}{non ho capito cosa sara' utile di questo, pero intanto appiccico quello che mi sembra utile} Let us formally define an incorrect coding proof, introducing also three key properties: accuracy, tightness and robustness, which allow us to compare different incorrect coding proofs.

\begin{Def}\label{def:bad} 
\textbf{Incorrect coding Proof Environment (BCPE)}
\\Let $A\subseteq \mathbb F_q^k\times \mathbb F_q^n$ be some set, which we call ambient.
Let $\code\subseteq \mathbb F_q^n$ be a linear code with dimension $k$, for which there exists an unambiguous procedure to pick a generator and a parity-check matrices $\6G$ and $\6H$. 
Let $W$ be some set with elements having a finite length binary representation, and ${\sf{Verify}}_{\hspace{-1mm}\scode}:D\times D\times W\mapsto\{{\sf{False}} \hspace{0.5mm};\hspace{0.5mm} {\sf{True}}\}$ be a function whose running time is polynomial in the input size. 
Then, we call $(\code,A,W,\verify)$ a incorrect coding Proof Environment (BCPE): $W$ is called witnesses space and the function $\verify$ is called relation. Let $(\6u,\6c)\in A$, and $h_u = {\mroot(\6u)}$ and $h_c = {\mroot(\6c)}$.
Then, we say that $w\in W$ is a witness for the pair $(h_u, h_c)$ if
$\verify(h_u,h_c,w) = {\sf{True}}$. \end{Def}

A malicious node has different ways to perform incorrect coding, and each strategy can be efficiently countered with ad-hoc strategies.
Then, any type of incorrect coding proof may work in some cases, but may not work in other cases.
In order to consider such possibilities, we have considered the notion of ambient, which contains all pairs $(\6u,\6c)$ to which a incorrect coding proof can be referred to.
In analogous way, different types of information may be required to provide the proof.
Hence, to embed all of such possibilities into a unique framework, we have defined the notion of witnesses space, which corresponds to the set of all the possible elements which can be furnished as a incorrect coding proof.
For example, in the cases in which the proof is provided as the original data itself, the witnesses space is constituted by the set of sequences with values in $\mathbb F_q$ and length $k$. 
Indeed, a re-encoding of the data would be enough to verify that the obtained codeword has a Merkle root which is different from the one in the header.
In analogous way, the procedure to verify the proof depends on the type of proof.
This feature is captured by the function $\verify$, which returns the value $\sf{True}$ when the header is incorrectly constructed. Let us define the following three properties. 

\begin{Def}\textbf{Accuracy}\label{def_accuracy}
\\Let $(\code,A,W,\verify)$ be a BCPE.
For $(h_u,h_c)\in D^2$, let $W_{h_u,h_c}\subseteq W$ be the set of all $w\in W$ such that $\verify(h_u,h_c,w) = {\sf{True}}$.
Then, we say that $(\code,A,W,{\sf{Verify}})$ is $\alpha$-accurate (or, equivalently, that it has accuracy $\alpha$) if 
$$\frac{\left|\left\{(\6u,\6c)\in A \mid W_{\mroot(\6u),\mroot(\6c)} = \varnothing\right\}\right|}{|A|} =  2^{-\alpha}.$$
\end{Def}
\begin{Def}\textbf{Tightness}\label{def_tightness}
\\Let $(\code,A,W,\verify)$ be a BCPE.
For $(\6u,\6c)\xleftarrow{\$} A$ and $h_u = \mroot(\6u)$, $h_c = \mroot(\6c)$, let $W_{h_u,h_c}\subseteq W$ be the set of all witnesses for the pair $(h_u,h_c)$. 
Then, we say that $(\code,A,W,\verify)$ is $\tau$-tight (or, equivalently, that it has tightness $\tau$) if $$\frac{|W_{h_u,h_c}|}{  |W|} =  2^{-\tau}.$$
\end{Def}
%\textcolor{red}{[FRANCO: La quantità tra parentesi graffe esprime, di fatto, una probabilità (approccio classico); è corretto? Non che lo si debba dichiarare; solo per chiarezza. ]}\textcolor{blue}{[yes. L'idea è proprio quella di capire con quale costo un attacco a forza bruta ti dà un witness. Si potrebbe definire tutto anche pensando all'advantage che un attaccante ha nel vincere il gioco di produrre un witness per una coppia di digests (come si fa per le proof di IND-CCA)... Solo che il tutto diventerebbe ancora più formale, astratto e... palloso. Magari teniamocelo buono per un paper successivo :)]}
\begin{Def}\textbf{Robustness}\label{def_robustness}
\\Let $(\code,A,W,\verify)$ be a BCPE. 
For $(h_u,h_c)\in D^2$, let $W_{h_u,h_c}\subseteq W$ be the set of all witnesses for the pair $(h_u,h_c)$. 
Let $\6u\rand \mathbb F_q^k$, 
$h_u = \mroot(\6u)$ and $h_c = \mroot(\6u\6G)$.
Then, we say that $(\code,A,W,{\sf{Verify}})$ is $\rho$-robust (or, equivalently, that it has robustness $\rho$) if 
$$\frac{|W_{h_u,h_c}|}{  |W|} =  2^{-\rho}.$$
\end{Def}


\end{comment}
